Constraining safe and unsafe overshoots in saddle-node bifurcations

We consider a dynamical system undergoing a saddle-node bifurcation with an explicitly time dependent parameter~$p(t)$. The combined dynamics can be considered as a dynamical systems where $p$ is a slowly evolving parameter. Here, we investigate settings where the parameter features an overshoot. It crosses the bifurcation threshold for some finite duration $t_e$ and up to an amplitude $R$, before it returns to its initial value. We denote the overshoot as safe when the dynamical system returns to its initial state. Otherwise, one encounters runaway trajectories (tipping), and the overshoot is unsafe. For shallow overshoots (small $R$) safe and unsafe overshoots are discriminated by an inverse square-root border, $t_e \propto R^{-1/2}$, as reported in earlier literature. However, for larger overshoots we here establish a crossover to another power law with an exponent that depends on the asymptotics of $p(t)$. For overshoots with a finite support we find that $t_e \propto R^{-1}$, and we provide examples for overshoots with exponents in the range $[-1, -1/2]$. All results are substantiated by numerical simulations, and it is discussed how the analytic and numeric results pave the way towards improved risks assessments separating safe from unsafe overshoots in climate, ecology and nonlinear dynamics.

==> Makefile <==
# SHELL = /bin/bash

FILE    = saddlenode
TALK    = saddlenode_vortrag
BIBS    = ${FILE}_bibliography.bib tipping.bib
FIGPATH = ./Sage/
FIGS = ${FIGPATH}overshoot_T-H.pdf ${FIGPATH}heterocline-jump__H_02.pdf  ${FIGPATH}heterocline-jump__H_50.pdf  ${FIGPATH}triangle-bound_lower.pdf  ${FIGPATH}triangle-bound_upper.pdf  ${FIGPATH}triangle_border.pdf  ${FIGPATH}sketch_bounds.pdf  ${FIGPATH}overshoot_Gauss_dc.pdf  ${FIGPATH}algebraic_large_d.pdf  ${FIGPATH}overshoot_c-d.pdf 



.PHONY: pdf clean

pdf: ${FILE}.tex ${FILE}.bbl ${FIGS}
	pdflatex ${FILE}.tex
	pdflatex ${FILE}.tex

${FILE}.bbl: ${BIBS} 
	pdflatex ${FILE}.tex
	-bibtex ${FILE}

Figures/%.pdf: Figures/%.svg Figures/texheader.tex
	echo $<
#	./makefig.sh $<
#epspdf figures/$(*F).pdf

tipping.bib: References/tipping.bib
	cp References/tipping.bib tipping.bib



clean:
	-rm -f *.aux *.bbl *.blg *.log *.out *.thm *.toc *.tdo *.bak *~ .*~ ${FILE}.dvi  *blx.bib *run.xml *.nav ${FILE}Notes.bib *.snm


SOURCE_PACKAGE_FILES = $(shell date +%y%m%d)_$(FILE).tgz
backup: 
	tar cvzf $(SOURCE_PACKAGE_FILES) --exclude="__BACKUP__/*" \
	Makefile README.md $(FILE).pdf $(FILE).tex  $(BIBS) \
	$(FIGPATH)*.pdf $(FIGPATH)*.ipynb
	mv $(SOURCE_PACKAGE_FILES) ./__BACKUP__/
	cp $(FILE).pdf  ./__BACKUP__/$(shell date +%y%m%d)_$(FILE).pdf

